Recurrence-in-Recurrence Networks for Video Deblurring

State-of-the-art video deblurring methods often adopt recurrent neural networks to model the temporal dependency between the frames. While the hidden states play key role in delivering information to the next frame, abrupt motion blur tend to weaken the relevance in the neighbor frames. In this paper, we propose recurrence-in-recurrence network architecture to cope with the limitations of short-ranged memory. We employ additional recurrent units inside the RNN cell. First, we employ inner-recurrence module (IRM) to manage the long-ranged dependency in a sequence. IRM learns to keep track of the cell memory and provides complementary information to find the deblurred frames. Second, we adopt an attention-based temporal blending strategy to extract the necessary part of the information in the local neighborhood. The adpative temporal blending (ATB) can either attenuate or amplify the features by the spatial attention. Our extensive experimental results and analysis validate the effectiveness of IRM and ATB on various RNN architectures.

==> sections/figs/fig_gopro_comparison.tex <==
\begin{figure}[t]
    \captionsetup[subfloat]{font=footnotesize}
    \centering
    \subfloat[Input blurry image]{\includegraphics[width=0.49\linewidth]{figs/figure5/blur.png}}
    \hfill
    \subfloat[Our deblurred image, RDBN+RIRN]{\includegraphics[width=0.49\linewidth]{figs/figure5/estrnn2.png}}
    \\
    %\vspace{-2mm}
    \subfloat[GRU]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/gru.png}}
    \hfill
    \subfloat[LSTM]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/lstm.png}}
    \hfill
    \subfloat[STRCNN~\cite{Kim_2017_ICCV}]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/strcnn.png}}
    \hfill
    \subfloat[IFIC1~\cite{Nah_2019_CVPR}]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/ific.png}}
    \hfill
    \subfloat[RDBN~\cite{zhong2020efficient}]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/estrnn.png}}
    \\
    \vspace{-2mm}
    \subfloat[GRU+RIRN]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/gru2.png}}
    \hfill
    \subfloat[LSTM+RIRN]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/lstm2.png}}
    \hfill
    \subfloat[STRCNN+RIRN]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/strcnn2.png}}
    \hfill
    \subfloat[IFIC1+RIRN]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/ific2.png}}
    \hfill
    \subfloat[RDBN+RIRN]{\includegraphics[width=0.19\textwidth]{figs/figure5/croped/estrnn2.png}}
    \figcspace
    \caption{Comparison of baselines and RIRN-applied method results in GOPRO~\cite{Nah_2017_CVPR} dataset}
    \label{fig:gopro_comparison}
    \figspace
\end{figure}
